Flaring gamma-ray emission coincident with a hyperactive fast radio burst source

Fast radio bursts (FRBs) are bright milliseconds-duration radio bursts from cosmological distances. Despite intense observational and theoretical studies, their physical origin is still mysterious. One major obstacle is the lack of identification of multi-wavelength counterparts for FRBs at cosmological distances. So far, all the searches other than in the radio wavelength, including those in the gamma-ray energies, have only left upper limits. Here we report a gigaelectronvolt (GeV) gamma-ray flare lasting 15.6 seconds as well as additional evidence of variable gamma-ray emission in temporal and spatial association with the hyper-active, newly discovered repeating FRB 20240114A, which has been localized to a dwarf galaxy at a redshift of 0.13. The energetic, short GeV gamma-ray flare reached a prompt isotropic luminosity of the order of ${10}^{48}~{\rm ergs~{s}^{-1}}$. The additional less-significant gamma-ray flares, if true, also have similar luminosities; such flares could contribute to a 5-day average luminosity of the order of ${10}^{45}~{\rm ergs~{s}^{-1}}$. These high-luminosity flares challenge the traditional FRB engine scenario involving a seconds-period magnetar. Rather, it suggests a powerful, long-lived, but newborn energy source at the location of this active repeater, either directly powering the bursts or indirectly triggering bursts in the vicinity of the FRB engine.

==> Ref2_old.tex <==
\begin{thebibliography}{34}
\setcounter{enumiv}{34}
\expandafter\ifx\csname url\endcsname\relax
  \def\url#1{\texttt{#1}}\fi
\expandafter\ifx\csname urlprefix\endcsname\relax\def\urlprefix{URL }\fi
\providecommand{\bibinfo}[2]{#2}
\providecommand{\eprint}[2][]{\url{#2}}

\bibitem{2020ApJS..247...33A}
\bibinfo{author}{{Abdollahi}, S.} \emph{et~al.}
\newblock \bibinfo{title}{{Fermi Large Area Telescope Fourth Source Catalog}}.
\newblock \emph{\bibinfo{journal}{\apjs}} \textbf{\bibinfo{volume}{247}},
  \bibinfo{pages}{33} (\bibinfo{year}{2020}).

\bibitem{mirabel94}
\bibinfo{author}{{Mirabel}, I.~F.} \& \bibinfo{author}{{Rodr{\'\i}guez}, L.~F.}
\newblock \bibinfo{title}{{A superluminal source in the Galaxy}}.
\newblock \emph{\bibinfo{journal}{\nat}} \textbf{\bibinfo{volume}{371}},
  \bibinfo{pages}{46--48} (\bibinfo{year}{1994}).

\bibitem{duncan92}
\bibinfo{author}{{Duncan}, R.~C.} \& \bibinfo{author}{{Thompson}, C.}
\newblock \bibinfo{title}{{Formation of Very Strongly Magnetized Neutron Stars:
  Implications for Gamma-Ray Bursts}}.
\newblock \emph{\bibinfo{journal}{\apjl}} \textbf{\bibinfo{volume}{392}},
  \bibinfo{pages}{L9} (\bibinfo{year}{1992}).

\bibitem{kluzniak98}
\bibinfo{author}{{Klu{\'z}niak}, W.} \& \bibinfo{author}{{Ruderman}, M.}
\newblock \bibinfo{title}{{The Central Engine of Gamma-Ray Bursters}}.
\newblock \emph{\bibinfo{journal}{\apjl}} \textbf{\bibinfo{volume}{505}},
  \bibinfo{pages}{L113--L117} (\bibinfo{year}{1998}).

\bibitem{dai06}
\bibinfo{author}{{Dai}, Z.~G.}, \bibinfo{author}{{Wang}, X.~Y.},
  \bibinfo{author}{{Wu}, X.~F.} \& \bibinfo{author}{{Zhang}, B.}
\newblock \bibinfo{title}{{X-ray Flares from Postmerger Millisecond Pulsars}}.
\newblock \emph{\bibinfo{journal}{Science}} \textbf{\bibinfo{volume}{311}},
  \bibinfo{pages}{1127--1129} (\bibinfo{year}{2006}).

\bibitem{lyubarsky14}
\bibinfo{author}{{Lyubarsky}, Y.}
\newblock \bibinfo{title}{{A model for fast extragalactic radio bursts.}}
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{442}},
  \bibinfo{pages}{L9--L13} (\bibinfo{year}{2014}).

\bibitem{metzger19}
\bibinfo{author}{{Metzger}, B.~D.}, \bibinfo{author}{{Margalit}, B.} \&
  \bibinfo{author}{{Sironi}, L.}
\newblock \bibinfo{title}{{Fast radio bursts as synchrotron maser emission from
  decelerating relativistic blast waves}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{485}},
  \bibinfo{pages}{4091--4106} (\bibinfo{year}{2019}).

\bibitem{beloborodov20}
\bibinfo{author}{{Beloborodov}, A.~M.}
\newblock \bibinfo{title}{{Blast Waves from Magnetar Flares and Fast Radio
  Bursts}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{896}},
  \bibinfo{pages}{142} (\bibinfo{year}{2020}).

\bibitem{lu20}
\bibinfo{author}{{Lu}, W.}, \bibinfo{author}{{Kumar}, P.} \&
  \bibinfo{author}{{Zhang}, B.}
\newblock \bibinfo{title}{{A unified picture of Galactic and cosmological fast
  radio bursts}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{498}},
  \bibinfo{pages}{1397--1405} (\bibinfo{year}{2020}).

\bibitem{cordes16}
\bibinfo{author}{{Cordes}, J.~M.} \& \bibinfo{author}{{Wasserman}, I.}
\newblock \bibinfo{title}{{Supergiant pulses from extragalactic neutron
  stars}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{457}},
  \bibinfo{pages}{232--257} (\bibinfo{year}{2016}).

\bibitem{luan14}
\bibinfo{author}{{Luan}, J.} \& \bibinfo{author}{{Goldreich}, P.}
\newblock \bibinfo{title}{{Physical Constraints on Fast Radio Bursts}}.
\newblock \emph{\bibinfo{journal}{\apjl}} \textbf{\bibinfo{volume}{785}},
  \bibinfo{pages}{L26} (\bibinfo{year}{2014}).

\bibitem{zhang14}
\bibinfo{author}{{Zhang}, B.}
\newblock \bibinfo{title}{{A Possible Connection between Fast Radio Bursts and
  Gamma-Ray Bursts}}.
\newblock \emph{\bibinfo{journal}{\apjl}} \textbf{\bibinfo{volume}{780}},
  \bibinfo{pages}{L21} (\bibinfo{year}{2014}).

\bibitem{wang24}
\bibinfo{author}{{Wang}, Y.}, \bibinfo{author}{{Zhang}, B.} \&
  \bibinfo{author}{{Zhu}, Z.}
\newblock \bibinfo{title}{{Anisotropic energy injection from magnetar central
  engines in short GRBs}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{528}},
  \bibinfo{pages}{3705--3718} (\bibinfo{year}{2024}).

\bibitem{zhang18}
\bibinfo{author}{{Zhang}, B.}
\newblock \bibinfo{title}{{FRB 121102: A Repeatedly Combed Neutron Star by a
  Nearby Low-luminosity Accreting Supermassive Black Hole}}.
\newblock \emph{\bibinfo{journal}{\apjl}} \textbf{\bibinfo{volume}{854}},
  \bibinfo{pages}{L21} (\bibinfo{year}{2018}).

\bibitem{ioka20}
\bibinfo{author}{{Ioka}, K.} \& \bibinfo{author}{{Zhang}, B.}
\newblock \bibinfo{title}{{A Binary Comb Model for Periodic Fast Radio
  Bursts}}.
\newblock \emph{\bibinfo{journal}{\apjl}} \textbf{\bibinfo{volume}{893}},
  \bibinfo{pages}{L26} (\bibinfo{year}{2020}).

\bibitem{anna-thomas23}
\bibinfo{author}{{Anna-Thomas}, R.} \emph{et~al.}
\newblock \bibinfo{title}{{Magnetic field reversal in the turbulent environment
  around a repeating fast radio burst}}.
\newblock \emph{\bibinfo{journal}{Science}} \textbf{\bibinfo{volume}{380}},
  \bibinfo{pages}{599--603} (\bibinfo{year}{2023}).
  
\end{thebibliography}


==> test2.tex <==
\begin{thebibliography}{10}
\setcounter{enumiv}{40}
\expandafter\ifx\csname url\endcsname\relax
  \def\url#1{\texttt{#1}}\fi
\expandafter\ifx\csname urlprefix\endcsname\relax\def\urlprefix{URL }\fi
\providecommand{\bibinfo}[2]{#2}
\providecommand{\eprint}[2][]{\url{#2}}

\bibitem{2017ApJ...846...98J}
\bibinfo{author}{{Jorstad}, S.~G.} \emph{et~al.}
\newblock \bibinfo{title}{{Kinematics of Parsec-scale Jets of Gamma-Ray Blazars
  at 43 GHz within the VLBA-BU-BLAZAR Program}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{846}},
  \bibinfo{pages}{98} (\bibinfo{year}{2017}).

\bibitem{2019ApJ...874...43L}
\bibinfo{author}{{Lister}, M.~L.} \emph{et~al.}
\newblock \bibinfo{title}{{MOJAVE. XVII. Jet Kinematics and Parent Population
  Properties of Relativistically Beamed Radio-loud Blazars}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{874}},
  \bibinfo{pages}{43} (\bibinfo{year}{2019}).

\bibitem{2019ARA&A..57..467B}
\bibinfo{author}{{Blandford}, R.}, \bibinfo{author}{{Meier}, D.} \&
  \bibinfo{author}{{Readhead}, A.}
\newblock \bibinfo{title}{{Relativistic Jets from Active Galactic Nuclei}}.
\newblock \emph{\bibinfo{journal}{\araa}} \textbf{\bibinfo{volume}{57}},
  \bibinfo{pages}{467--509} (\bibinfo{year}{2019}).

\bibitem{1992Natur.358..215M}
\bibinfo{author}{{Mirabel}, I.~F.}, \bibinfo{author}{{Rodriguez}, L.~F.},
  \bibinfo{author}{{Cordier}, B.}, \bibinfo{author}{{Paul}, J.} \&
  \bibinfo{author}{{Lebrun}, F.}
\newblock \bibinfo{title}{{A double-sided radio jet from the compact Galactic
  Centre annihilator 1E1740.7-2942}}.
\newblock \emph{\bibinfo{journal}{\nat}} \textbf{\bibinfo{volume}{358}},
  \bibinfo{pages}{215--217} (\bibinfo{year}{1992}).

\bibitem{2004ARA&A..42..317F}
\bibinfo{author}{{Fender}, R.} \& \bibinfo{author}{{Belloni}, T.}
\newblock \bibinfo{title}{{GRS 1915+105 and the Disc-Jet Coupling in Accreting
  Black Hole Systems}}.
\newblock \emph{\bibinfo{journal}{\araa}} \textbf{\bibinfo{volume}{42}},
  \bibinfo{pages}{317--364} (\bibinfo{year}{2004}).

\bibitem{1972_ApJ}
\bibinfo{author}{{Matilsky}, T.~A.}, \bibinfo{author}{{Giacconi}, R.},
  \bibinfo{author}{{Gursky}, H.}, \bibinfo{author}{{Kellogg}, E.~M.} \&
  \bibinfo{author}{{Tananbaum}, H.~D.}
\newblock \bibinfo{title}{{A New Transient Source Observed by UHURU}}.
\newblock \emph{\bibinfo{journal}{\apjl}} \textbf{\bibinfo{volume}{174}},
  \bibinfo{pages}{L53--L55} (\bibinfo{year}{1972}).

\bibitem{1984_PASJ}
\bibinfo{author}{{Kitamoto}, S.}, \bibinfo{author}{{Miyamoto}, S.},
  \bibinfo{author}{{Tsunemi}, H.}, \bibinfo{author}{{Makishima}, K.} \&
  \bibinfo{author}{{Nakagawa}, M.}
\newblock \bibinfo{title}{{The transient X-ray source 4U 1543-47 observed from
  Tenma.}}
\newblock \emph{\bibinfo{journal}{\pasj}} \textbf{\bibinfo{volume}{36}},
  \bibinfo{pages}{799--806} (\bibinfo{year}{1984}).

\bibitem{1992_IAUC}
\bibinfo{author}{{Harmon}, B.~A.} \emph{et~al.}
\newblock \bibinfo{title}{{U 1543-47}}.
\newblock \emph{\bibinfo{journal}{\iaucirc}} \textbf{\bibinfo{volume}{5510}},
  \bibinfo{pages}{2} (\bibinfo{year}{1992}).

\bibitem{2002_IAUC}
\bibinfo{author}{{Miller}, J.~M.} \& \bibinfo{author}{{Remillard}, R.~A.}
\newblock \bibinfo{title}{{4U 1543-47}}.
\newblock \emph{\bibinfo{journal}{\iaucirc}} \textbf{\bibinfo{volume}{7920}},
  \bibinfo{pages}{2} (\bibinfo{year}{2002}).

\bibitem{2003_IAUS_Orosz}
\bibinfo{author}{{Orosz}, J.~A.}
\newblock \bibinfo{title}{{Inventory of black hole binaries}}.
\newblock In \emph{\bibinfo{booktitle}{A Massive Star Odyssey: From Main
  Sequence to Supernova}}, vol. \bibinfo{volume}{212}, \bibinfo{pages}{365}
  (\bibinfo{year}{2003}).
\newblock \eprint{astro-ph/0209041}.

\bibitem{2002_AAS_Orosz}
\bibinfo{author}{{Orosz}, J.~A.} \emph{et~al.}
\newblock \bibinfo{title}{{Revised parameters for the black hole binary 4U
  1543-47}}.
\newblock In \emph{\bibinfo{booktitle}{American Astronomical Society Meeting
  Abstracts}}, vol. \bibinfo{volume}{201} of \emph{\bibinfo{series}{American
  Astronomical Society Meeting Abstracts}}, \bibinfo{pages}{15.11}
  (\bibinfo{year}{2002}).

\bibitem{2003_A&A_Ritter}
\bibinfo{author}{{Ritter}, H.} \& \bibinfo{author}{{Kolb}, U.}
\newblock \bibinfo{title}{{Catalogue of cataclysmic binaries, low-mass X-ray
  binaries and related objects (Seventh edition)}}.
\newblock \emph{\bibinfo{journal}{\aap}} \textbf{\bibinfo{volume}{404}},
  \bibinfo{pages}{301--303} (\bibinfo{year}{2003}).

\bibitem{2023ApJ...946...19D}
\bibinfo{author}{{Draghis}, P.~A.} \emph{et~al.}
\newblock \bibinfo{title}{{A Systematic View of Ten New Black Hole Spins}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{946}},
  \bibinfo{pages}{19} (\bibinfo{year}{2023}).

\bibitem{2020MNRAS.493.4409D}
\bibinfo{author}{{Dong}, Y.}, \bibinfo{author}{{Garc{\'\i}a}, J.~A.},
  \bibinfo{author}{{Steiner}, J.~F.} \& \bibinfo{author}{{Gou}, L.}
\newblock \bibinfo{title}{{The spin measurement of the black hole in 4U 1543-47
  constrained with the X-ray reflected emission}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{493}},
  \bibinfo{pages}{4409--4417} (\bibinfo{year}{2020}).

\bibitem{2006ApJ...636L.113S}
\bibinfo{author}{{Shafee}, R.} \emph{et~al.}
\newblock \bibinfo{title}{{Estimating the Spin of Stellar-Mass Black Holes by
  Spectral Fitting of the X-Ray Continuum}}.
\newblock \emph{\bibinfo{journal}{\apjl}} \textbf{\bibinfo{volume}{636}},
  \bibinfo{pages}{L113--L116} (\bibinfo{year}{2006}).

\bibitem{2009PASJ}
\bibinfo{author}{{Matsuoka}, M.} \emph{et~al.}
\newblock \bibinfo{title}{{The MAXI Mission on the ISS: Science and Instruments
  for Monitoring All-Sky X-Ray Images}}.
\newblock \emph{\bibinfo{journal}{\pasj}} \textbf{\bibinfo{volume}{61}},
  \bibinfo{pages}{999} (\bibinfo{year}{2009}).

\bibitem{2009IEEEP_Jonas}
\bibinfo{author}{{Jonas}, J.~L.}
\newblock \bibinfo{title}{{MeerKAT - The South African Array With Composite
  Dishes and Wide-Band Single Pixel Feeds}}.
\newblock \emph{\bibinfo{journal}{IEEE Proceedings}}
  \textbf{\bibinfo{volume}{97}}, \bibinfo{pages}{1522--1530}
  (\bibinfo{year}{2009}).

\bibitem{fender2017thunderkat}
\bibinfo{author}{Fender, R.} \emph{et~al.}
\newblock \bibinfo{title}{Thunderkat: The meerkat large survey project for
  image-plane radio transients} (\bibinfo{year}{2017}).
\newblock \eprint{1711.04132}.

\bibitem{2004ApJ_Gehrels}
\bibinfo{author}{{Gehrels}, N.} \emph{et~al.}
\newblock \bibinfo{title}{{The Swift Gamma-Ray Burst Mission}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{611}},
  \bibinfo{pages}{1005--1020} (\bibinfo{year}{2004}).

\bibitem{2004MNRAS.355.1105F}
\bibinfo{author}{{Fender}, R.~P.}, \bibinfo{author}{{Belloni}, T.~M.} \&
  \bibinfo{author}{{Gallo}, E.}
\newblock \bibinfo{title}{{Towards a unified model for black hole X-ray binary
  jets}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{355}},
  \bibinfo{pages}{1105--1118} (\bibinfo{year}{2004}).

\bibitem{2004MNRAS.347L..52G}
\bibinfo{author}{{Gallo}, E.}, \bibinfo{author}{{Corbel}, S.},
  \bibinfo{author}{{Fender}, R.~P.}, \bibinfo{author}{{Maccarone}, T.~J.} \&
  \bibinfo{author}{{Tzioumis}, A.~K.}
\newblock \bibinfo{title}{{A transient large-scale relativistic radio jet from
  GX 339-4}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{347}},
  \bibinfo{pages}{L52--L56} (\bibinfo{year}{2004}).

\bibitem{2022ApJS..260...12W}
\bibinfo{author}{{Weaver}, Z.~R.} \emph{et~al.}
\newblock \bibinfo{title}{{Kinematics of Parsec-scale Jets of Gamma-Ray Blazars
  at 43 GHz during 10 yr of the VLBA-BU-BLAZAR Program}}.
\newblock \emph{\bibinfo{journal}{\apjs}} \textbf{\bibinfo{volume}{260}},
  \bibinfo{pages}{12} (\bibinfo{year}{2022}).

\bibitem{2002ApJ...569..362S}
\bibinfo{author}{{Smith}, D.~M.}, \bibinfo{author}{{Heindl}, W.~A.} \&
  \bibinfo{author}{{Swank}, J.~H.}
\newblock \bibinfo{title}{{Two Different Long-Term Behaviors in Black Hole
  Candidates: Evidence for Two Accretion Flows?}}
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{569}},
  \bibinfo{pages}{362--380} (\bibinfo{year}{2002}).

\bibitem{2004ApJ...611L.121Y}
\bibinfo{author}{{Yu}, W.}, \bibinfo{author}{{van der Klis}, M.} \&
  \bibinfo{author}{{Fender}, R.}
\newblock \bibinfo{title}{{The Correlation between Hard X-Ray Peak Flux and
  Soft X-Ray Peak Flux in the Outburst Rise of Low-Mass X-Ray Binaries}}.
\newblock \emph{\bibinfo{journal}{\apjl}} \textbf{\bibinfo{volume}{611}},
  \bibinfo{pages}{L121--L124} (\bibinfo{year}{2004}).

\bibitem{2007ApJ...663.1309Y}
\bibinfo{author}{{Yu}, W.}, \bibinfo{author}{{Lamb}, F.~K.},
  \bibinfo{author}{{Fender}, R.} \& \bibinfo{author}{{van der Klis}, M.}
\newblock \bibinfo{title}{{Peak Luminosities of the Hard States of GX 339-4:
  Implications for the Accretion Geometry, Disk Mass, and Black Hole Mass}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{663}},
  \bibinfo{pages}{1309--1314} (\bibinfo{year}{2007}).

\bibitem{2007A&A_Evans}
\bibinfo{author}{{Evans}, P.~A.} \emph{et~al.}
\newblock \bibinfo{title}{{An online repository of Swift/XRT light curves of
  {\ensuremath{\gamma}}-ray bursts}}.
\newblock \emph{\bibinfo{journal}{\aap}} \textbf{\bibinfo{volume}{469}},
  \bibinfo{pages}{379--385} (\bibinfo{year}{2007}).

\bibitem{2009MNRAS_Evans}
\bibinfo{author}{{Evans}, P.~A.} \emph{et~al.}
\newblock \bibinfo{title}{{Methods and results of an automatic analysis of a
  complete sample of Swift-XRT observations of GRBs}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{397}},
  \bibinfo{pages}{1177--1201} (\bibinfo{year}{2009}).

\bibitem{1996ASPC_Arnaud}
\bibinfo{author}{{Arnaud}, K.~A.}
\newblock \bibinfo{title}{{XSPEC: The First Ten Years}}.
\newblock In \bibinfo{editor}{{Jacoby}, G.~H.} \& \bibinfo{editor}{{Barnes},
  J.} (eds.) \emph{\bibinfo{booktitle}{Astronomical Data Analysis Software and
  Systems V}}, vol. \bibinfo{volume}{101} of
  \emph{\bibinfo{series}{Astronomical Society of the Pacific Conference
  Series}}, \bibinfo{pages}{17} (\bibinfo{year}{1996}).

\bibitem{2016A&A_HI4PI}
\bibinfo{author}{{HI4PI Collaboration}} \emph{et~al.}
\newblock \bibinfo{title}{{HI4PI: A full-sky H I survey based on EBHIS and
  GASS}}.
\newblock \emph{\bibinfo{journal}{\aap}} \textbf{\bibinfo{volume}{594}},
  \bibinfo{pages}{A116} (\bibinfo{year}{2016}).

\bibitem{Remillard_2022}
\bibinfo{author}{Remillard, R.~A.} \emph{et~al.}
\newblock \bibinfo{title}{An empirical background model for the {NICER} x-ray
  timing instrument}.
\newblock \emph{\bibinfo{journal}{The Astronomical Journal}}
  \textbf{\bibinfo{volume}{163}}, \bibinfo{pages}{130} (\bibinfo{year}{2022}).
\newblock \urlprefix\url{https://doi.org/10.3847%2F1538-3881%2Fac4ae6}.

\bibitem{2007ASPC_McMullin}
\bibinfo{author}{{McMullin}, J.~P.}, \bibinfo{author}{{Waters}, B.},
  \bibinfo{author}{{Schiebel}, D.}, \bibinfo{author}{{Young}, W.} \&
  \bibinfo{author}{{Golap}, K.}
\newblock \bibinfo{title}{{CASA Architecture and Applications}}.
\newblock In \bibinfo{editor}{{Shaw}, R.~A.}, \bibinfo{editor}{{Hill}, F.} \&
  \bibinfo{editor}{{Bell}, D.~J.} (eds.) \emph{\bibinfo{booktitle}{Astronomical
  Data Analysis Software and Systems XVI}}, vol. \bibinfo{volume}{376} of
  \emph{\bibinfo{series}{Astronomical Society of the Pacific Conference
  Series}}, \bibinfo{pages}{127} (\bibinfo{year}{2007}).

\bibitem{2020ascl.soft_oxkat}
\bibinfo{author}{{Heywood}, I.}
\newblock \bibinfo{title}{{oxkat: Semi-automated imaging of MeerKAT
  observations}}.
\newblock \bibinfo{howpublished}{Astrophysics Source Code Library, record
  ascl:2009.003} (\bibinfo{year}{2020}).
\newblock \eprint{2009.003}.

\bibitem{1995PhDT.......238B}
\bibinfo{author}{{Briggs}, D.~S.}
\newblock \emph{\bibinfo{title}{{High fidelity deconvolution of moderately
  resolved sources}}}.
\newblock Ph.D. thesis, \bibinfo{school}{New Mexico Institute of Mining and
  Technology} (\bibinfo{year}{1995}).

\bibitem{2010MNRAS.402.2403M}
\bibinfo{author}{{Murphy}, T.} \emph{et~al.}
\newblock \bibinfo{title}{{The Australia Telescope 20 GHz Survey: the source
  catalogue}}.
\newblock \emph{\bibinfo{journal}{\mnras}} \textbf{\bibinfo{volume}{402}},
  \bibinfo{pages}{2403--2423} (\bibinfo{year}{2010}).

\bibitem{2016ApJ...821...61P}
\bibinfo{author}{{Partridge}, B.} \emph{et~al.}
\newblock \bibinfo{title}{{Absolute Calibration of the Radio Astronomy Flux
  Density Scale at 22 to 43 GHz Using Planck}}.
\newblock \emph{\bibinfo{journal}{\apj}} \textbf{\bibinfo{volume}{821}},
  \bibinfo{pages}{61} (\bibinfo{year}{2016}).

\bibitem{2018A&A_GaiaDR2}
\bibinfo{author}{{Gaia Collaboration}} \emph{et~al.}
\newblock \bibinfo{title}{{Gaia Data Release 2. Summary of the contents and
  survey properties}}.
\newblock \emph{\bibinfo{journal}{\aap}} \textbf{\bibinfo{volume}{616}},
  \bibinfo{pages}{A1} (\bibinfo{year}{2018}).

\bibitem{2003ApJ...589L..33Y}
\bibinfo{author}{{Yu}, W.}, \bibinfo{author}{{Klein-Wolt}, M.},
  \bibinfo{author}{{Fender}, R.} \& \bibinfo{author}{{van der Klis}, M.}
\newblock \bibinfo{title}{{Hard X-Ray Flares Preceding Soft X-Ray Outbursts in
  Aquila X-1: A Link between Neutron Star and Black Hole State Transitions}}.
\newblock \emph{\bibinfo{journal}{\apjl}} \textbf{\bibinfo{volume}{589}},
  \bibinfo{pages}{L33--L36} (\bibinfo{year}{2003}).

\end{thebibliography}

